BRUM: Robust 3D Vehicle Reconstruction from 360 Sparse Images

Accurate 3D reconstruction of vehicles is vital for applications such as vehicle inspection, predictive maintenance, and urban planning. Existing methods like Neural Radiance Fields and Gaussian Splatting have shown impressive results but remain limited by their reliance on dense input views, which hinders real-world applicability. This paper addresses the challenge of reconstructing vehicles from sparse-view inputs, leveraging depth maps and a robust pose estimation architecture to synthesize novel views and augment training data. Specifically, we enhance Gaussian Splatting by integrating a selective photometric loss, applied only to high-confidence pixels, and replacing standard Structure-from-Motion pipelines with the DUSt3R architecture to improve camera pose estimation. Furthermore, we present a novel dataset featuring both synthetic and real-world public transportation vehicles, enabling extensive evaluation of our approach. Experimental results demonstrate state-of-the-art performance across multiple benchmarks, showcasing the method's ability to achieve high-quality reconstructions even under constrained input conditions.

==> Sections/6_references.tex <==
\section*{References}

% Please number citations consecutively within brackets \cite{b1}. The 
% sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
% number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
% the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

% Number footnotes separately in superscripts. Place the actual footnote at 
% the bottom of the column in which it was cited. Do not put footnotes in the 
% abstract or reference list. Use letters for table footnotes.

% Unless there are six authors or more give all authors' names; do not use 
% ``et al.''. Papers that have not been published, even if they have been 
% submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
% that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
% Capitalize only the first word in a paper title, except for proper nouns and 
% element symbols.

% For papers published in translation journals, please give the English 
% citation first, followed by the original foreign-language citation \cite{b6}.

% \begin{thebibliography}{00}
% \bibitem{b1} B. Mildenhall, P.P. Srinivasan, M. Tancik, J.T. Barron, R. Ramamoorthi, R. Ng: ``Nerf: Representing scenes as neural radiance fields for view synthesis'', Communications of the ACM, 65(1), 2021.
% \bibitem{b2} B. Kerbl, G. Kopanas, T. Leimkühler, G. Drettakis: ``3D Gaussian Splatting for Real-Time Radiance Field Rendering'', ACM Trans. Graph., 42(4), 2023.
% \bibitem{b3} D. Di Nucci, A. Simoni, M. Tomei, L. Ciuffreda, R. Vezzani, R. Cucchiara: ``Carpatch: A synthetic benchmark for radiance field evaluation on vehicle components''. ICIAP, 2023.
% \bibitem{b4} D. Di Nucci, A. Simoni, M. Tomei, L. Ciuffreda, R. Vezzani, R. Cucchiara: ``KRONC: Keypoint-based Robust Camera Optimization for 3D Car Reconstruction'', ECCV Workshops, 2024.
% \bibitem{b5} A. Tonderski, C. Lindström, G. Hess, W. Ljungbergh, L. Svensson, C. Petersson: ``Neurad: Neural rendering for autonomous driving'', CVPR, 2024.
% \bibitem{b6} X. Zhou, Z. Lin, X. Shan, Y. Wang, D. Sun, M. H. Yang: ``DrivingGaussian: Composite Gaussian splatting for surrounding dynamic autonomous driving scenes'', CVPR, 2024.
% \bibitem{b7} H. Turki, D. Ramanan, M. Satyanarayanan: ``Mega-nerf: Scalable construction of large-scale nerfs for virtual fly-throughs'', CVPR, 2022.
% \bibitem{b8} H. Xie, Z. Chen, F. Hong, Z. Liu: ``Citydreamer: Compositional generative model of unbounded 3D cities'', CVPR, 2024.
% \bibitem{b9} Y. Liu, C. Luo, L. Fan, N. Wang, J. Peng, Z. Zhang: ``CityGaussian: Real-time high-quality large-scale scene rendering with Gaussians'', ECCV, 2024.
% \bibitem{b10} P. Truong, M. J. Rakotosaona, F. Manhardt, F. Tombari: ``Sparf: Neural radiance fields from sparse and noisy poses'', CVPR, 2023.
% \bibitem{b11} J. L. Schonberger, J. M. Frahm, ``Structure-from-motion revisited'', CVPR 2016.
% \bibitem{b12} S. Wang, V. Leroy, Y. Cabon, B. Chidlovskii, J. Revaud: ``Dust3r: Geometric 3D vision made easy'', CVPR, 2024.
% \bibitem{b13} T. Müller, A. Evans, C. Schied, A. Keller: ``Instant neural graphics primitives with a multiresolution hash encoding''. ACM TOG, 2022.
% \bibitem{b14} S. Fridovich-Keil, A. Yu, M. Tancik, Q. Chen, B. Recht, A. Kanazawa: ``Plenoxels: Radiance fields without neural networks'', CVPR, 2022.
% \bibitem{b15} A. Chen, Z. Xu, A. Geiger, J. Yu, H. Su: ``Tensorf: Tensorial radiance fields'', ECCV, 2022.
% \bibitem{b16} C. H. Lin, W. C. Ma, A. Torralba, S. Lucey: ``Barf: Bundle-adjusting neural radiance fields'', ICCV, 2021.
% \bibitem{b17} Y. Chen, X. Chen, X. Wang, Q. Zhang, Y. Guo, Y. Shan, F. Wang: ``Local-to-global registration for bundle-adjusting neural radiance fields'', CVPR, 2023.
% \bibitem{b18} W. Bian, Z. Wang, K. Li, J. W. Bian, V. A. Prisacariu: ``Nope-nerf: Optimising neural radiance field with no pose prior'', CVPR, 2023.
% \bibitem{b19} S. Chen, Y. Bhalgat, X. Li, J. W. Bian, K. Li, Z. Wang, V. A. Prisacariu: ``Neural Refinement for Absolute Pose Regression with Feature Synthesis'', CVPR, 2024.
% \bibitem{b20} W. Morgenstern, F. Barthel, A. Hilsmann, P. Eisert: ``Compact 3D scene representation via self-organizing Gaussian grids'', ECCV, 2024.
% \bibitem{b21} S. Niedermayr, J. Stumpfegger, R. Westermann: ``Compressed 3D Gaussian splatting for accelerated novel view synthesis'', CVPR, 2024.
% \bibitem{b22} Z. Fan, K. Wang, K. Wen, Z. Zhu, D. Xu, Z. Wang: ``LightGaussian: Unbounded 3D Gaussian compression with 15x reduction and 200+ fps'', NeurIPS, 2024.
% \bibitem{b23} X. Zhang, X. Ge, T. Xu, D. He, Y. Wang, H. Qin, G. Lu, J. Geng, J. Zhang: ``Gaussianimage: 1000 fps image representation and compression by 2D Gaussian splatting'', ECCV, 2024.
% \bibitem{b24} J. Cen, Z. Zhou, J. Fang, W. Shen, L. Xie, D. Jiang, X. Zhang, Q. Tian: ``Segment anything in 3D with NeRFs'', NeurIPS, 2023.
% \bibitem{b25} X. Hu, Y. Wang, L. Fan, J. Fan, J. Peng, Z. Lei, L. Qing, Z. Zhang: ``Segment anything in 3D Gaussians'', arXiv preprint, 2024.
% \bibitem{b26} Y. Chen, Z. Chen, C. Zhang, F. Wang, X. Yang, Y. Wang, Z. Cai, L. Yang, H. Liu, G. Lin: ``Gaussianeditor: Swift and controllable 3D editing with Gaussian splatting'', CVPR, 2024.
% \bibitem{b27} S. Zhou, Z. Fan, D. Xu, H. Chang, P. Chari, T. Bharadwaj, S. You, Z. Wang,A. Kadambi: ``Dreamscene360: Unconstrained text-to-3D scene generation with panoramic Gaussian splatting'', ECCV, 2024.
% \bibitem{b28} Z. Chen, F. Wang, Y. Wang, H. Liu: ``Text-to-3D using Gaussian splatting'', CVPR, 2024.
% \bibitem{b29} Y. Liang, X. Yang, J. Lin, H. Li, X. Xu, Y. Chen: ``LucidDreamer: Towards high-fidelity text-to-3D generation via interval score matching'', CVPR, 2024.


% \bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% \bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% \bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% \bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% \bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
% \bibitem{b8} D. P. Kingma and M. Welling, ``Auto-encoding variational Bayes,'' 2013, arXiv:1312.6114. [Online]. Available: https://arxiv.org/abs/1312.6114
% \bibitem{b9} S. Liu, ``Wi-Fi Energy Detection Testbed (12MTC),'' 2023, gitHub repository. [Online]. Available: https://github.com/liustone99/Wi-Fi-Energy-Detection-Testbed-12MTC
% \bibitem{b10} ``Treatment episode data set: discharges (TEDS-D): concatenated, 2006 to 2009.'' U.S. Department of Health and Human Services, Substance Abuse and Mental Health Services Administration, Office of Applied Studies, August, 2013, DOI:10.3886/ICPSR30122.v2
% \bibitem{b11} K. Eves and J. Valasek, ``Adaptive control for singularly perturbed systems examples,'' Code Ocean, Aug. 2023. [Online]. Available: https://codeocean.com/capsule/4989235/tree
\end{thebibliography}

==> Tables/efficiency.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}
\begin{table}[t]
\centering
\caption{Runtime and GPU memory consumption for each method. The Data are reported considering a single run on the \textit{Jeep} scene of CarPatch dataset \textcolor{red}{rivedi come grafico}}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c}
\toprule 
\textbf{Method} & \textbf{Runtime} & \textbf{GPU Memory} \\
\midrule
3DGS~\cite{} & 4 min & 4.5 GB \\
\rowcolor{myrowcolor}
DNGaussians~\cite{} & 4 min & 4.5 GB \\
SplatFields~\cite{} & 3 hours & 5.4 GB \\
\rowcolor{myrowcolor}
\method~\cite{} & 14 min & 4.5 GB \\
\bottomrule
\end{tabular}}
\label{tab:time_mem}
%\vspace{-.5cm}
\end{table}
